ToolTweak: An Attack on Tool Selection in LLM-based Agents

As LLMs increasingly power agents that interact with external tools, tool use has become an essential mechanism for extending their capabilities. These agents typically select tools from growing databases or marketplaces to solve user tasks, creating implicit competition among tool providers and developers for visibility and usage. In this paper, we show that this selection process harbors a critical vulnerability: by iteratively manipulating tool names and descriptions, adversaries can systematically bias agents toward selecting specific tools, gaining unfair advantage over equally capable alternatives. We present ToolTweak, a lightweight automatic attack that increases selection rates from a baseline of around 20% to as high as 81%, with strong transferability between open-source and closed-source models. Beyond individual tools, we show that such attacks cause distributional shifts in tool usage, revealing risks to fairness, competition, and security in emerging tool ecosystems. To mitigate these risks, we evaluate two defenses: paraphrasing and perplexity filtering, which reduce bias and lead agents to select functionally similar tools more equally. All code will be open-sourced upon acceptance.

==> tables/OLD-defended-results-tsr.tex <==
\begin{tabular}{|l|c|c|c|c|c|}
\hline
 & DeepSeek & Gemini & GPT-OSS & Llama 3.1 & Qwen 2.5 \\
\hline
Attack & 48.64 ($\color{red}{\downarrow32.98}$) & 30.16 ($\color{red}{\downarrow18.50}$) & 63.30 ($\color{red}{\downarrow10.32}$) & 27.24 ($\color{red}{\downarrow6.72}$) & 34.30 ($\color{red}{\downarrow11.62}$) \\
Manual Suffix & 30.20 ($\color{red}{\downarrow51.42}$) & 21.32 ($\color{red}{\downarrow27.34}$) & 37.50 ($\color{red}{\downarrow36.12}$) & 20.44 ($\color{red}{\downarrow13.52}$) & 32.76 ($\color{red}{\downarrow13.16}$) \\
\hline
\end{tabular}


==> tables/OLD-main-results-tsr.tex <==
\begin{tabular}{|l|r|r|r|r|r|}
\hline
 & DeepSeek & Gemini & GPT-OSS & Llama 3.1 & Qwen 2.5 \\
\hline
No Attack & 20.16 & 18.86 & 18.96 & 19.84 & 19.90 \\
Attack & \textbf{81.62} & 48.66 & 73.62 & 33.96 & 45.92 \\
Manual Suffix & 68.66 & \textbf{56.10} & \textbf{76.44} & \textbf{38.12} & \textbf{61.26} \\
\hline
\end{tabular}

==> tables/defended-results-tsr.tex <==
% \begin{tabular}{|l|l||c|c|c|c|c|c|}
% \hline
%  &  & DeepSeek & Gemini & GPT-OSS & Grok 3 Mini & Llama 3.1 & Qwen 2.5 \\
% \hline
% \multirow[t]{2}{*}{Attack} & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
%  & Defended & 48.6 & 30.1 & 63.3 & 32.7 & 27.2 & 34.3 \\
% \cline{1-8}
% Attack Against Defender & Defended & 59.7 & 37.5 & 67.9 & 44.8 & 34.4 & 46.7 \\
% \cline{1-8}
% \multirow[t]{2}{*}{Manual Suffix} & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\
%  & Defended & 30.2 & 21.3 & 37.5 & 22.7 & 20.4 & 32.7 \\
% \cline{1-8}
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \cline{1-8}
% \hline
% \end{tabular}

% \begin{xltabular}{\textwidth}{|l|l||c|c|c|c|c|c|}

% \hline
%  &  & DeepSeek & Gemini & GPT-OSS & Grok 3 & Llama 3.1 & Qwen 2.5 \\
% &  &  & & & Mini &  &  \\
% \hline
% \multirow[t]{2}{*}{Attack} & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
%  & Defended & 48.6 & 30.1 & 63.3 & 32.7 & 27.2 & 34.3 \\
% \cline{1-8}
% Attacking & \multirow[t]{2}{*}{Defended} & \multirow[t]{2}{*}{59.7} & \multirow[t]{2}{*}{37.5} & \multirow[t]{2}{*}{67.9} & \multirow[t]{2}{*}{44.8} & \multirow[t]{2}{*}{34.4} & \multirow[t]{2}{*}{46.7} \\
% Defended &  &  & &  &  &  &  \\
% \cline{1-8}
% \multirow[t]{2}{*}{Manual Suffix} & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\
%  & Defended & 30.2 & 21.3 & 37.5 & 22.7 & 20.4 & 32.7 \\
% \cline{1-8}
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \cline{1-8}
% \hline
% \end{xltabular}


% \begin{xltabular}{\textwidth}{llccXXXX}
% \hline 
%  &  & DeepSeek & Gemini & GPT-OSS & Grok3 Mini & Llama 3.1 & Qwen 2.5 \\
% \cline{1-8}
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \cline{1-8}
% \multirow[t]{2}{*}{Attack} & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
% & Defended \rowcolor{lightgray}  & 48.6 & 30.1 & 63.3 & 32.7 & 27.2 & 34.3 \\
% \cline{1-8}
% Attacking Defended & Defended \rowcolor{lightgray} & 59.7 & 37.5 & 67.9 & 44.8 & 34.4 & 46.7 \\
% \cline{1-8}
% \multirow[t]{2}{*}{Manual Suffix} & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\

% & Defended \rowcolor{lightgray} & 30.2 & 21.3 & 37.5 & 22.7 & 20.4 & 32.7 \\
% \hline
% \end{xltabular}


% \begin{xltabular}{\textwidth}{llccXXXX}
% \hline 
%  &  & DeepSeek & Gemini & GPT-OSS & Grok3 Mini & Llama 3.1 & Qwen 2.5 \\
% \cline{1-8}
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \hline
% \multirow[t]{2}{*}{Attack} & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
%  & \cellcolor[gray]{.9} Defended & \cellcolor[gray]{.9} 48.6 & \cellcolor[gray]{.9} 30.1 & \cellcolor[gray]{.9} 63.3 & \cellcolor[gray]{.9} 32.7 & \cellcolor[gray]{.9} 27.2 & \cellcolor[gray]{.9} 34.3 \\  \hline



% Attacking Defended & \cellcolor[gray]{.9} Defended & \cellcolor[gray]{.9} 59.7 & \cellcolor[gray]{.9} 37.5 & \cellcolor[gray]{.9} 67.9 & \cellcolor[gray]{.9} 44.8 & \cellcolor[gray]{.9} 34.4 & \cellcolor[gray]{.9} 46.7 \\
% \hline
% \multirow[t]{2}{*}{Manual Suffix} & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\

% & \cellcolor[gray]{.9} Defended & \cellcolor[gray]{.9} 30.2 & \cellcolor[gray]{.9} 21.3 & \cellcolor[gray]{.9} 37.5 & \cellcolor[gray]{.9} 22.7 & \cellcolor[gray]{.9} 20.4 & \cellcolor[gray]{.9} 32.7 \\
% \hline
% \end{xltabular}


% \begin{table}[t]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2} % more row height
% \begin{tabularx}{\textwidth}{llccXXXX}
% \toprule
%  &  & \textbf{DeepSeek} & \textbf{Gemini} & \textbf{GPT-OSS} & \textbf{Grok3 Mini} & \textbf{Llama 3.1} & \textbf{Qwen 2.5} \\
% \midrule
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \midrule
% \multirow[t]{2}{*}{\centering Attack} 
%   & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
%   & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 48.6 & \cellcolor{lightgray} 30.1 & \cellcolor{lightgray} 63.3 & \cellcolor{lightgray} 32.7 & \cellcolor{lightgray} 27.2 & \cellcolor{lightgray} 34.3 \\  
% \midrule
% Attacking Defended & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 59.7 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 67.9 & \cellcolor{lightgray} 44.8 & \cellcolor{lightgray} 34.4 & \cellcolor{lightgray} 46.7 \\
% \midrule
% \multirow[t]{2}{*}{\centering Manual Suffix} 
%   & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\
%   & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 30.2 & \cellcolor{lightgray} 21.3 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 22.7 & \cellcolor{lightgray} 20.4 & \cellcolor{lightgray} 32.7 \\
% \bottomrule
% \end{tabularx}
% \caption{Results of different models under various attacks and defenses.}
% \end{table}

% \begin{table}[t]
% \footnotesize
% \centering
% \renewcommand{\arraystretch}{1.2} % more row height
% \begin{tabular}{llcccccc}
% \toprule
%  &  & \textbf{DeepSeek} & \textbf{Gemini} & \textbf{GPT-OSS} & \textbf{Grok3 Mini} & \textbf{Llama 3.1} & \textbf{Qwen 2.5} \\
% \midrule
% No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
% \midrule
% % \multirow[t]{2}{*}{\centering Attack} 
% \multirow[c]{2}{*}{Attack}
%   & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
%   & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 48.6 & \cellcolor{lightgray} 30.1 & \cellcolor{lightgray} 63.3 & \cellcolor{lightgray} 32.7 & \cellcolor{lightgray} 27.2 & \cellcolor{lightgray} 34.3 \\  
% \midrule
% Attacking Defended & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 59.7 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 67.9 & \cellcolor{lightgray} 44.8 & \cellcolor{lightgray} 34.4 & \cellcolor{lightgray} 46.7 \\
% \midrule
% \multirow[t]{2}{*}{\centering Manual Suffix} 
%   & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\
%   & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 30.2 & \cellcolor{lightgray} 21.3 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 22.7 & \cellcolor{lightgray} 20.4 & \cellcolor{lightgray} 32.7 \\
% \bottomrule
% \end{tabular}
% \caption{Results of different models under various attacks and defenses.}
% \end{table}

\begin{table}[t]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llcccccc}
\toprule
 &  & \textbf{DeepSeek} & \textbf{Gemini} & \textbf{GPT-OSS} & \textbf{Grok3 Mini} & \textbf{Llama 3.1} & \textbf{Qwen 2.5} \\
\midrule
No Attack & Undefended & 20.1 & 18.8 & 18.9 & 19.9 & 19.8 & 19.9 \\
\midrule
\multirow[c]{2}{*}{Attack}
  & Undefended & 81.6 & 48.6 & 73.6 & 50.7 & 33.9 & 45.9 \\
  & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 48.6 & \cellcolor{lightgray} 30.1 & \cellcolor{lightgray} 63.3 & \cellcolor{lightgray} 32.7 & \cellcolor{lightgray} 27.2 & \cellcolor{lightgray} 34.3 \\
\midrule
Attacking Defended & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 59.7 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 67.9 & \cellcolor{lightgray} 44.8 & \cellcolor{lightgray} 34.4 & \cellcolor{lightgray} 46.7 \\
\midrule
% Remove \centering here; use [c] and (optional) \multicolumn to center horizontally
\multirow[c]{2}{*}{\multicolumn{1}{c}{Manual Suffix}}
  & Undefended & 68.6 & 56.1 & 76.4 & 89.4 & 38.1 & 61.2 \\
  & \cellcolor{lightgray} Defended & \cellcolor{lightgray} 30.2 & \cellcolor{lightgray} 21.3 & \cellcolor{lightgray} 37.5 & \cellcolor{lightgray} 22.7 & \cellcolor{lightgray} 20.4 & \cellcolor{lightgray} 32.7 \\
\bottomrule
\end{tabular}
\caption{Results of different models under various attacks and defenses.}
\end{table}

==> tables/main-results-tsr.tex <==
% \begin{tabularx}{\textwidth}{Xcccccc}
% \hline 
%  & DeepSeek & Gemini & GPT-OSS & Grok 3 Mini & Llama 3.1 & Qwen 2.5 \\
% \cline{2-7}
% No Attack & 20.16 & 18.86 & 18.96 & 19.94 & 19.84 & 19.90 \\
% Attack & \textbf{81.62} & 48.66 & 73.62 & 50.74 & 33.96 & 45.92 \\
% \multirow[t]{2}{*}{Manual Suffix} & 68.66 & \textbf{56.10} & \textbf{76.44} & \textbf{89.46} & \textbf{38.12} & \textbf{61.26} \\
% \hline
% \end{tabularx}


% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2} % row height
% \begin{tabularx}{\textwidth}{lcccccc}
% \toprule
%  & \textbf{DeepSeek} & \textbf{Gemini} & \textbf{GPT-OSS} & \textbf{Grok 3 Mini} & \textbf{Llama 3.1} & \textbf{Qwen 2.5} \\
% \midrule
% No Attack & 20.16 & 18.86 & 18.96 & 19.94 & 19.84 & 19.90 \\
% Attack & \textbf{81.62} & 48.66 & 73.62 & 50.74 & 33.96 & 45.92 \\
% Manual Suffix & 68.66 & \textbf{56.10} & \textbf{76.44} & \textbf{89.46} & \textbf{38.12} & \textbf{61.26} \\
% \bottomrule
% \end{tabularx}
% \caption{Comparison of models on different conditions (higher is worse).}
% \end{table}
